Location Privacy and Spectrum Efficiency Enhancement in Spectrum Sharing Systems

In this work, we investigate the benefits of secondary user (SU) network beamforming on improving primary user (PU) location privacy in spectrum sharing systems, where the beamformer in the SU network is designed to suppress the aggregate interference to improve the location privacy of PUs. We consider two problems: improving SU network communication throughput subject to the specified PU location privacy requirements, and enhancing PU location privacy given the quality of service (QoS) requirements of SU networks. In the first problem, we provide an algorithm to achieve high data rates with the constrained PU location privacy level. Numerical results show that for a given PU location privacy requirement, the proposed scheme is able to interfere/exclude only a few SU nodes from the PU band and the network throughput can be greatly improved. In the second problem, to fully explore the potential of SU network beamforming for enhancing PU location privacy, we propose a two-step scheme to decouple the beamforming and privacy zone design so that the PU location privacy can be improved while satisfying the SU network throughput requirement. According to numerical evaluations, the proposed scheme can maintain/achieve higher PU location privacy than the benchmark beamforming schemes while satisfying a QoS requirement for the SU network.

==> Complexity.tex <==
\vspace{-1cm}
\subsection{Computational Complexity Analysis}
\label{Complexity}

In this section, we evaluate the computational complexity of the proposed solutions to the three problems. As will be
shown in the numerical results, the proposed algorithms exhibit
gains in terms of both convergence and performance compared to the conventional MRC-based schemes. Now, we will present the complexity comparison by adopting the analysis in \cite{zhu2017beamforming,zhu2016outage}. Here, we denote $n$, and $Q_{\text{max}}$ as the number of decision variables and SCA iteration number, respectively.  In the privacy zone design problem, it involves
1 SOC of dimension $|\mathcal{C}_r|$ and $9MN+|\mathcal{C}_r|$
linear constraints. For the aggregate interference reduction problem, it contains $2$ SOC constraint with the same dimension $MN$, and $2MN$ linear constraints. 

%For the algorithm of data rate maximization under the location privacy constraint, the SOCP is solved using the SCA algorithm. In this algorithm, 3 SOC constriants with the size of $MN$ are established. It has $7MN+2W$ linear constraints.


\begin{table*}[t]
  \caption{COMPLEXITY ANALYSIS OF DIFFERENT ALGORITHMS}
  \centering
  \begin{tabular}{|p{4.5cm}||c|}
      \hline
    \textbf{Algorithms} & \textbf{Complexity Order} \\
    \hline
    SU data rate maximization under the PU location privacy constraint & $\mathcal{O}(n\mathcal{Q}^{\text{max}}\sqrt{7MN+2W+6}\big[3(MN)^2+7MN+2W+n^2\big])$, where $n=\mathcal{O}(3+8MN+2W)$\\
    \hline
    Step 1: privacy zone design algorithm &  $\mathcal{O}(n\mathcal{Q}^{\text{max}}\sqrt{|\mathcal{C}_r|+9MN+2}\big[|\mathcal{C}_r|^2+9MN+|\mathcal{C}_r|+n^2\big])$, where $n=\mathcal{O}(9MN+1+2|\mathcal{C}_r|)$\\
    \hline
    Step 2: aggregate interference reduction & $\mathcal{O}(n\mathcal{Q}^{\text{max}}\sqrt{2MN+6}\big[3(MN)^2+2MN+n^2\big])$, where $n=\mathcal{O}(3+3MN)$\\
    \hline
  \end{tabular}
  \label{tab:1}
\end{table*}



==> Problem_formulation.tex <==
\section{Optimal Solutions}

\subsection{Problem Transformation}

\begin{lem}
For the ZF beamformer, the constraints on the spectrum efficiency are equivalent to the constraint as below:
\begin{eqnarray}
p_{m,n}\geq \sigma_{m,n}^2(2^{r_{m,n}}-1){u_{m,n}}
\label{ERTS_34r}
\end{eqnarray}
\label{SSERT_34}
\end{lem}
\begin{proof}
Let $\gamma_{m,n}=\frac{|\tilde{\bf{h}}_{m,n}^H{\bf{w}}_{m,n}|^2u_{m,n}p_{m,n}}{I_{inter}^{m}+I_{intra}+\sigma_{m,n}^2}$. The first constraint can be reformulated as ${1+\gamma_{m,n}}{\geq 2^{u_{m,n}r_{m,n}}}$。This term is able to be decoupled into $\gamma_{m,n}\geq(2^{r_{m,n}})^{u_{m,n}}-1$. The range of term $(2^{r_{m,n}})^{u_{m,n}}-1$ is discrete, which is within $\in\{0,2^{r_{m,n}}-1\}$. Based on this observation, the equation above is able to be regrouped into $\gamma_{m,n}\geq(2^{r_{m,n}}-1){u_{m,n}}$. For the ZF beamformer, SNR $\gamma_{m,n}$ can be simplified into $\gamma_{m,n}=\frac{p_{m,n}u_{m,n}}{\sigma_{m,n}^2}$. To this end, the transformation for the first constraint is achieved. 
\label{RTSTY_32}
\end{proof}

\begin{lem}
The transform of constraints on the aggregated interference is given as:
\begin{eqnarray}
\tilde{I}_{m,n}^{i,j}u_{m,n}{{p}}_{m,n}{\geq 10^{ I_{th}/10-3}(1-v_{i,j})}
\label{RTYS_456}
\end{eqnarray}
\label{RTSI_234}
\end{lem}
\begin{proof}
The Eq. \ref{SS_rty23} can be transformed into
\begin{eqnarray}
\Big(10\text{log}_{10}(\sum_{m}\sum_{n}I_{m,n}^{i,j}u_{m,n})\Big)\leq (I_{th}-30)
\label{ERTS_123}
\end{eqnarray}
To prevent the aggregated interference from exceeding the interference threshold, the following inequality still holds:
\begin{eqnarray}
(\sum_{m,n}I_{m,n}^{i,j}u_{m,n})\geq 10^{(I_{th}-30)/10}(1-v_{i,j})
\label{ERTS_123}
\end{eqnarray}
The derivation in Eq.\ref{ERTS_123} decouples the linear multiplication, which is critical for our problem.
\end{proof}
Gathering all of results from the two lemmas above, the original problem can be transformed into:
\begin{maxi!}[2]
	{v_{i,j},u_{m,n},p_{m,n}}{{\sum_i\sum_j v_{i,j}}}
	{}{}\label{sss_45}	\addConstraint{u_{m,n}p_{m,n}}{\geq \sigma_{m,n}^2(2^{r_{m,n}}-1){u_{m,n}}
}
	\addConstraint{\sum_{m,n}I_{m,n}^{i,j}u_{m,n}}{\geq 10^{I_{th}/10-3}(1-v_{i,j})}
	\addConstraint{\sum_{n}u_{m,n}p_{m,n}}{\leq P_m}
	\addConstraint{\forall m\in\mathcal{M},~\forall n \in\mathcal{N}_m}{}
	\addConstraint{v_{i,j}}{\in\{0,1\}}
	\addConstraint{u_{m,n}}{\in\{0,1\}}
	%\label{sss_45}
\end{maxi!}
\subsection{Problem Relaxation}
\begin{lem}
To further simplify the problem above, an extra constraint \cite{ZhiqiangWei} can be introduced:
\begin{eqnarray}
p_{m,n}=u_{m,n}p_{m,n},~\forall m,n
\label{RTY_YSE}
\end{eqnarray}
\end{lem}
The constraint above is still intractable. According to \cite{Weizhiqiang,Other}, a penalty term can be incorporated into the objective function to handle the constraint in Eq. \ref{RTY_YSE}.



